Improving Query Representations for Dense Retrieval with Pseudo Relevance Feedback

Dense retrieval systems conduct first-stage retrieval using embedded representations and simple similarity metrics to match a query to documents. Its effectiveness depends on encoded embeddings to capture the semantics of queries and documents, a challenging task due to the shortness and ambiguity of search queries. This paper proposes ANCE-PRF, a new query encoder that uses pseudo relevance feedback (PRF) to improve query representations for dense retrieval. ANCE-PRF uses a BERT encoder that consumes the query and the top retrieved documents from a dense retrieval model, ANCE, and it learns to produce better query embeddings directly from relevance labels. It also keeps the document index unchanged to reduce overhead. ANCE-PRF significantly outperforms ANCE and other recent dense retrieval systems on several datasets. Analysis shows that the PRF encoder effectively captures the relevant and complementary information from PRF documents, while ignoring the noise with its learned attention mechanism.

==> arxiv/01_intro.tex <==
\section{Introduction}

\cx{
Intro outline:
\begin{enumerate}
    \item p1: the advancement of dense retrieval and the potential of it
    \item p2: query representation is hard as query is short, encoder has little context, the challenges in query understanding also persists in representation learning. E.g. in LeR having the doc fixed and continues train the query rep can lead to better performance
    \item p3: A classic IR technique is leverage PRF to improve q representation. in sparse retrieval it is to find terms to expand the query.
    \item p4: In this paper, we investigate and show the advantage of PRF in improve DR.  We uses a new PRF encoder, that takes the q and PRF doc, and learns to produce a better query representation.  Benefit from DR is end-to-end trainable, we directly train the prf encoder from final relevance label, using ANCE. In addition, we keep doc representation from the DR model untouched to avoid duplicating index for PRF
    \item p5: Our exp on MARCO passage, TREC DL, show ANCE-PRF significantly improves its DR model, ANCE. It outperforms various recent STOA on these and also MARCO passage leaderboard. 
    \item p6: analyse show that PRF does provide better query representation, in the space, getting closer to relevance doc and also q with relevance feedback. further study shows the PRF-Encoder learns to pay more attention to terms in the relevance PRF doc, and especially terms that are important compensation to the short query. We will release code and data for future research.
\end{enumerate}}


Large pre-trained Transformer~\cite{transformer} language models~\cite{bert,gpt2,gpt3,deberta,t5} been successful on various retrieval benchmark datasets~\cite{msmarco,trecdl19,trecdl20}. A common pipeline of Transformer-based retrieval systems involves a fast initial retrieval stage using bag-of-words model such as BM25~\cite{bm25,deepct}, followed by a Transformer re-ranker~\cite{monobert}. However, the re-ranking stage usually involves evaluating hundreds of query-document pairs on the neural model, incurring latency that is too high for real-world production. 

To facilitate more efficient neural retrieval systems, recent research have been exploring dense retrieval systems. In dense retrieval, document encoding is moved to offline indexing time, and fast nearest neighbor search on query-document similarity is utilized to expedite online retrieval. However, the retrieval time query encoding is usually a standalone procedure, where the query encoder reads a sole query as the input. The query encoder is hence not able to utilize the intricate relevance information from the learned document embedding space for refined query representations. 

\hc{Some discussion on previous work?} 

In this work, we propose a pseudo relevance feedback (PRF) method to improve query representations in dense retrieval, which we name ANCE-PRF. Our method aims to guide the query encoder using the high quality top-retrieved documents from ANCE~\cite{ance}, a recent dense retriever. Specifically, ANCE-PRF provides a query encoder that takes as input a combination of the query and the feedback documents, and it is able to produce query embeddings that reflect both the original query and the selected feedback relevance information. 

This work makes the following contributions to the study of PRF and dense retrieval
\begin{itemize}
    \item To the best of our knowledge, ANCE-PRF is the first attempt to study PRF in dense retrieval. 
    \item We show that ANCE-PRF is an effective framework \hc{by framework I intend to say that it can be used with other dense retrievers as well. Currently this idea is not mentioned} that can significantly improve the retrieval performance over the underlying dense retriever. 
    \item We analyze ANCE-PRF's attention distribution and learned query embedding space, and we show that ANCE-PRF effectively learns to recognize feedback relevance information. 
\end{itemize}

\hc{1. Currently the introduction looks like a simple expansion of the abstract. There might be some more insights to be added; 2. More references?} 
